RMP screening in JOREK-CARIDDI

Edge localized modes (ELMs) are instabilities at the tokamak edge that can have short outbursts of highly energetic particles and heat, which can severely damage the walls of a plasma reactor. Resonant magnetic perturbations (RMPs) are used to mitigate or eliminate ELMs from the plasma. One effect that can reduce the intensity of the RMP is screening, which is caused by eddy currents in conducting structures or a plasma that are induced by a time-varying magnetic field. The eddy current code CARIDDI was recently coupled with the magnetohydrodynamics (MHD) code JOREK, and is able to capture the behavior of volumetric conducting structures that surround a plasma. The objective of this study is to characterize screening behavior in the JOREK-CARIDDI coupling. The analysis is divided in three parts. First, CARIDDI results are benchmarked against results from STARWALL, another JOREK extension that captures interactions of (two-dimensional) conducting structures. It is found that CARIDDI and STARWALL show good agreement, with slight variations. The second part covers the screening of time-varying RMP fields by conducting structures, oscillating at frequencies from 3 Hz to 10 kHz. The overall trends in screening behavior align qualitatively with findings from a previous analysis. However, an additional contribution to the screening at frequencies above 1 kHz was not observed, because the simulation in this report does not include screening by the RMP coil casing. Finally, a few tests were performed using a plasma configuration, to study the effect of plasma screening, including realistic plasma background flows. The results demonstrated the induction of eddy currents at rational surfaces within the plasma. These results contribute to an improved understanding of the screening of RMP fields, which is relevant for several applications to the operation of fusion reactors.

==> TEMP/Settings/packages.tex <==
\usepackage{a4wide}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage[toc,page]{appendix}
\usepackage[english]{babel}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{blindtext}
\usepackage[font=it]{caption}
\usepackage{esint}
\usepackage{eurosym}
\usepackage{fancyhdr}
\usepackage{float}
\usepackage[margin=1.0in]{geometry}
\usepackage{graphicx}
\RequirePackage{doi}
\usepackage{hyperref}
\usepackage[utf8]{inputenc}
\usepackage{listings}
\usepackage{makecell}
\usepackage{mathtools}
\usepackage{multirow}
%\usepackage[square,numbers]{natbib}
\usepackage[intoc]{nomencl}
\usepackage[parfill]{parskip}
\usepackage{rotating}
\usepackage{siunitx}
\usepackage{tikz}
\usepackage{titlesec}
\usepackage{upgreek}
\usepackage{url}
\usepackage{verbatim}
\usepackage{xfrac}
\usepackage{xparse}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{tcolorbox}
\usepackage{lipsum}
\tcbuselibrary{breakable}
%geen idee
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{color}

%memes
\usepackage{wallpaper} 

\usepackage{calligra}\usepackage{a4wide}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage[toc,page]{appendix}
\usepackage[english]{babel}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{blindtext}
\usepackage[font=it]{caption}
\usepackage{esint}
\usepackage{eurosym}
\usepackage{fancyhdr}
\usepackage{float}
\usepackage[margin=1.0in]{geometry}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage[utf8]{inputenc}
\usepackage{listings}
\usepackage{makecell}
\usepackage{mathtools}
\usepackage{multirow}
%\usepackage[square,numbers]{natbib}
\usepackage[intoc]{nomencl}
\usepackage[parfill]{parskip}
%\usepackage{physics}
\usepackage{rotating}
\usepackage{siunitx}
\usepackage{tikz}
\usepackage{titlesec}
\usepackage{upgreek}
\usepackage{url}
\usepackage{verbatim}
\usepackage{xfrac}
\usepackage{xparse}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{tcolorbox}
\usepackage{lipsum}
\tcbuselibrary{breakable}
%geen idee
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{color}

\usepackage{calligra}
\usepackage{comment}

\usepackage[nottoc]{tocbibind}
\usepackage{amsmath}
\everydisplay{\centering}
\usepackage[export]{adjustbox}

==> TEMP/Settings/titlepage.tex <==
\title{
	\begin{center}
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.4\textwidth]{TEMP/Settings/Nikhef-logo-RGB-red-on-white-500x225.png}
	\end{figure}
	
	\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{TEMP/Settings/RU_Logo.png}
         %\caption{$y=x$}
         %\label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{TEMP/Settings/TUe-logo-scarlet-rgb.png}
         %\caption{$y=3sinx$}
         %\label{fig:three sin x}
     \end{subfigure}

\end{figure}
	
    \huge{The neutrino - lepton production angle at high energies} \\[0.2cm]
    \Huge{\bfseries master thesis} \\
    \line(1,0){450} \\ [2cm]
\end{center}
}



\author{
    \textit{} \\
	\begin{tabular}{rcl}
        Bas Slotema & s1073279 (RU)/1233729 (TU/e)\\
	\end{tabular} \\[0.5cm]
	}


\date\today

==> TEMP/chapters/Outlook.tex <==
\chapter{Outlook}
\label{chap:outlook}

